Scalable, Time-Responsive, Digital, Energy-Efficient Molecular Circuits using DNA Strand Displacement

We propose a novel theoretical biomolecular design to implement any Boolean circuit using the mechanism of DNA strand displacement. The design is scalable: all species of DNA strands can in principle be mixed and prepared in a single test tube, rather than requiring separate purification of each species, which is a barrier to large-scale synthesis. The design is time-responsive: the concentration of output species changes in response to the concentration of input species, so that time-varying inputs may be continuously processed. The design is digital: Boolean values of wires in the circuit are represented as high or low concentrations of certain species, and we show how to construct a single-input, single-output signal restoration gate that amplifies the difference between high and low, which can be distributed to each wire in the circuit to overcome signal degradation. This means we can achieve a digital abstraction of the analog values of concentrations. Finally, the design is energy-efficient: if input species are specified ideally (meaning absolutely 0 concentration of unwanted species), then output species converge to their ideal concentrations at steady-state, and the system at steady-state is in (dynamic) equilibrium, meaning that no energy is consumed by irreversible reactions until the input again changes. Drawbacks of our design include the following. If input is provided non-ideally (small positive concentration of unwanted species), then energy must be continually expended to maintain correct output concentrations even at steady-state. In addition, our fuel species - those species that are permanently consumed in irreversible reactions - are not "generic"; each gate in the circuit is powered by its own specific type of fuel species. Hence different circuits must be powered by different types of fuel. Finally, we require input to be given according to the dual-rail convention, so that an input of 0 is specified not only by the absence of a certain species, but by the presence of another. That is, we do not construct a "true NOT gate" that sets its output to high concentration if and only if its input's concentration is low. It remains an open problem to design scalable, time-responsive, digital, energy-efficient molecular circuits that additionally solve one of these problems, or to prove that some subset of their resolutions are mutually incompatible.

==> conclusion.tex <==
\section{Conclusion}
\label{sec-conclusion}


==> figures/amplification.tex <==
\pspicture(-0.5,-0.5)(14,8.5)
  \rput[lb](5.25,0.35){$x$}\psline(5,0.25)(6,0.25)\pstAMP(6,0)
  \rput[lb](6.5,0.35){$a_1$}\psline(6.5,0.25)(7,0.25)\pstAMP(7,0)
  \rput[lb](7.5,0.35){$a_2$}\psline(7.5,0.25)(8,0.25)\pstAMP(8,0)
  \rput[lb](8.5,0.35){$a_3$}\psline(8.5,0.25)(9,0.25)
  \rput(7,-0.5){(a)}
  
  \rput[lb](0,2){\psscalebox{0.4}{\epsfbox{figures/amp_abs.eps}}} 
  \rput(4,1.5){(b)} \rput(6,1.8){\psscalebox{0.75}{Time}}\rput{90}(-0.25,7){\psscalebox{0.75}{Concentration}}
  \rput[lb](6.0,7.8){\psscalebox{0.8}{$x$}}
  \rput[lb](6.0,7.45){\psscalebox{0.8}{$a_1$}}
  \rput[lb](6.0,7.1){\psscalebox{0.8}{$a_2$}}
  \rput[lb](6.0,6.78){\psscalebox{0.8}{$a_3$}}


  \rput[lb](7,2){\psscalebox{0.5}{\epsfbox{figures/amp.eps}}} 
  \rput(10.5,1.5){(c)} \rput(13,1.8){\psscalebox{0.75}{Time}}
  \rput[lb](1.75,-0.2){
    \rput[lb](13.0,7.8){\psscalebox{0.8}{$x$}}
    \rput[lb](13.0,7.45){\psscalebox{0.8}{$a_1$}}
    \rput[lb](13.0,7.1){\psscalebox{0.8}{$a_2$}}
    \rput[lb](13.0,6.78){\psscalebox{0.8}{$a_3$}}
  }
\endpspicture



==> figures/dflipflop.tex <==
\pspicture(-1,0.75)(18,8)
  \rput[lb](3,3.5){
    \pstAMP(0,0.5)\pstNAND(1,0) \pstFANOUT(3,0.1)
    \pstAMP(0,2)\pstNAND(1,2) \pstFANOUT(3,2.1)
    \pstNAND(-2,-0.25)\pstNAND(-2,2.25)
    \pstFANOUT(-3,1.1)
    \pstFANOUT(-6.3,2.4)\pstNAND(-4.5,-0.5)\pstFANOUT(-5.5,-0.4)

    \psline(-0.6,0.25)(1,0.25)
    \psline(2.4,0.5)(3,0.5)
    \psline(3.4,0.3)(4.5,0.3)\rput[lb](4,0.4){$\neg Q$}
    \psline(3.4,0.7)(3.6,0.7)(3.6,1)(-0.2,1.95)(-0.2,2.25)(0,2.25)
    \psline(0.5,2.25)(1,2.25)

    \psline(-0.6,2.75)(1,2.75)
    \psline(2.4,2.5)(3,2.5)
    \psline(3.4,2.7)(4.5,2.7)\rput[lb](4.25,2.8){$Q$}
    \psline(3.4,2.3)(3.6,2.3)(3.6,2)(-0.2,1.05)(-0.2,0.75)(0,0.75)
    \psline(0.5,0.75)(1,0.75)

    \rput[lb](-4,1.6){clock}\psline(-4,1.5)(-3,1.5)\psline(-2.6,1.3)(-2.3,1.3)(-2.3,0.5)(-2,0.5)\psline(-2.6,1.7)(-2.3,1.7)(-2.3,2.5)(-2,2.5)

    \rput[lb](-6.8,2.9){$D$}\psline(-6.8,2.8)(-6.3,2.8)\psline(-5.9,3)(-2,3)\psline(-5.9,2.6)(-5.7,2.6)(-5.7,0)(-5.5,0)
    \psline(-5.1,-0.2)(-4.5,-0.2)\psline(-5.1,0.2)(-4.5,0.2)\psline(-3.1,0)(-2,0)
    \rput(2,-2){(a3)}
  }
  \rput[lb](9,0){
    \rput[lb](0,2){\psscalebox{0.5}{\epsfbox{figures/dflipflop_abs.eps}}} 
    \rput(5,1.5){(b3)} \rput(8,1.8){\psscalebox{0.75}{Time}}\rput{90}(-0.25,7){\psscalebox{0.75}{Concentration}}
  }
\endpspicture



==> figures/gate-shapes.tex <==
\usepackage{pstricks}

\newcommand{\NORblock}{%
  \begin{pspicture}(0.5,1){%
      \psarc(0,.5){.5}{270}{90}}
  \end{pspicture}%
}

\makeatletter
\def\pstFANOUT{\pst@object{pstFANOUT}}
\def\pstFANOUT@i(#1){{%
  \begin@ClosedObj
  \rput[lb](#1){%
    \pspolygon(0,0)(0,0.8)(0.4,0.8)(0.4,0)}
  \end@ClosedObj}%
  \ignorespaces%
}
\def\pstAMP{\pst@object{pstAMP}}
\def\pstAMP@i(#1){{%
  \begin@ClosedObj
  \rput[lb](#1){%
    \pspolygon(0,0)(0,0.5)(0.5,0.25)}
  \end@ClosedObj}%
  \ignorespaces%
}
\def\pstNOR{\pst@object{pstNOR}}
\def\pstNOR@i(#1){{%
  \begin@ClosedObj
  \rput[lb](#1){%
    \psscaleboxto(1.2,1){\NORblock}%
    \pscircle(0.1,0.5){0.1} 
  }
  \rput[lb](#1){%
    \psscaleboxto(0.3,1){\NORblock}}
  \end@ClosedObj}%
  \ignorespaces%
}
\def\pstNAND{\pst@object{pstNAND}}
\def\pstNAND@i(#1){{%
  \begin@ClosedObj
  \rput[lb](#1){%
    \psscaleboxto(1.2,1){\NORblock}%
    \pscircle(0.1,0.5){0.1} 
  }
  \rput[lb](#1){%
    \psline(0,0)(0,1)}
  \end@ClosedObj}%
  \ignorespaces%
}
\makeatother


==> figures/latch.tex <==
\pspicture(-1,-4)(18,8)
  \rput[lb](7.5,-3){
    \pstAMP(0,0.5)\pstNOR(1,0) \pstFANOUT(3,0.1)
    \pstAMP(0,2)\pstNOR(1,2) \pstFANOUT(3,2.1)

    \psline(-0.75,0.25)(1.25,0.25)\rput[lb](-0.75,0.35){$S$}
    \psline(2.4,0.5)(3,0.5)
    \psline(3.4,0.3)(4.5,0.3)\rput[lb](4,0.4){$\neg Q$}
    \psline(3.4,0.7)(3.6,0.7)(3.6,1)(-0.2,1.95)(-0.2,2.25)(0,2.25)
    \psline(0.5,2.25)(1.25,2.25)

    \psline(-0.75,2.75)(1.25,2.75)\rput[lb](-0.75,2.85){$R$}
    \psline(2.4,2.5)(3,2.5)
    \psline(3.4,2.7)(4.5,2.7)\rput[lb](4.25,2.8){$Q$}
    \psline(3.4,2.3)(3.6,2.3)(3.6,2)(-0.2,1.05)(-0.2,0.75)(0,0.75)
    \psline(0.5,0.75)(1.25,0.75)
    \rput(2,-0.5){(a)}
  }
  \rput[lb](0,2){\psscalebox{0.5}{\epsfbox{figures/latch_abs.eps}}} 
  \rput(5,1.5){(b)} \rput(8,1.8){\psscalebox{0.75}{Time}}\rput{90}(-0.25,7){\psscalebox{0.75}{Concentration}}

  \rput[lb](9,2){\psscalebox{0.5}{\epsfbox{figures/latch.eps}}} 
  \rput(13.5,1.5){(c)} \rput(17,1.8){\psscalebox{0.75}{Time}}
\endpspicture



==> figures/moderate.tex <==
\pspicture(0,0)(18,8)
  \rput[lb](0,2){\psscalebox{0.5}{\epsfbox{figures/moderate_abs.eps}}} 
  \rput(5,1.5){(b2)} \rput(8,1.8){\psscalebox{0.75}{Time}}\rput{90}(-0.25,7){\psscalebox{0.75}{Concentration}}
  \rput[lb](8.4,6.65){
    \rput[lb](0,0.81){\psscalebox{0.8}{$x$}}
    \rput[lb](0,0.54){\psscalebox{0.8}{$y$}}
    \rput[lb](0,0.27){\psscalebox{0.8}{$z$}}
    \rput[lb](0,0){\psscalebox{0.8}{$o$}}
  }

  \rput[lb](9,2){\psscalebox{0.58}{\epsfbox{figures/moderate.eps}}} 
  \rput(13.5,1.5){(c2)} \rput(17,1.8){\psscalebox{0.75}{Time}}
  \rput[lb](18.6,6.7){
    \rput[lb](0,0.75){\psscalebox{0.8}{$x$}}
    \rput[lb](0,0.5){\psscalebox{0.8}{$y$}}
    \rput[lb](0,0.25){\psscalebox{0.8}{$z$}}
    \rput[lb](0,0){\psscalebox{0.8}{$o$}}
  }



\endpspicture



==> figures/nand-amp.tex <==
\pspicture(-1,-4)(18,8)
  \rput[lb](9.5,-3){
    \pstFANOUT(1,1)
    \pstNAND(2,0)
    \pstNAND(2,2)
    \pstAMP(4,0.25)
    \pstAMP(4,2.25)
    \pstNAND(5.5,1)

    \rput[lb](0,1.5){$y$}\psline(0,1.4)(1,1.4)
    \psline(1.4,1.2)(1.7,1.2)(1.7,0.75)(2,0.75)\psline(1.4,1.6)(1.7,1.6)(1.7,2.25)(2,2.25)
    \rput[lb](0,2.85){$x$}\psline(0,2.75)(2,2.75)
    \rput[lb](0,0.35){$z$}\psline(0,0.25)(2,0.25)
    \psline(3.4,0.5)(4,0.5)\psline(4.5,0.5)(5,0.5)(5,1.25)(5.5,1.25)
    \psline(3.4,2.5)(4,2.5)\psline(4.5,2.5)(5,2.5)(5,1.75)(5.5,1.75)
    \psline(6.9,1.5)(7.5,1.5)\rput[rb](7.5,1.6){$o$}

    \rput(4,-0.5){(a2)}
  }

  \rput[lb](3,-1.95){
    \pstNAND(1,0)
    \pstAMP(3,0.25)
    
    \rput[lb](0,0.35){$y$}\psline(0,0.25)(1,0.25)
    \rput[lb](0,0.85){$x$}\psline(0,0.75)(1,0.75)
    \psline(2.4,0.5)(3,0.5)\psline(3.5,0.5)(4.5,0.5)

    \rput(2,-1.5){(a1)}
  }
  \rput[lb](0,2){\psscalebox{0.5}{\epsfbox{figures/nand_amp_abs.eps}}} 
  \rput(5,1.5){(b1)} \rput(8,1.8){\psscalebox{0.75}{Time}}\rput{90}(-0.25,7){\psscalebox{0.75}{Concentration}}

  \rput[lb](9,2){\psscalebox{0.5}{\epsfbox{figures/nand_amp.eps}}} 
  \rput(13.5,1.5){(c1)} \rput(17,1.8){\psscalebox{0.75}{Time}}

\endpspicture



==> toeholds.tex <==
\opt{dnasubmission}{
\section{Toeholds, Linkers, and Buffers}}
\opt{normal}{
\subsection{Toeholds, Linkers, and Buffers}}
\label{sec-toeholds-linkers-buffers}

\opt{dnasubmission}{
\subsection{Preventing Crosstalk between Linkers}}
\opt{normal}{
\subsubsection{Preventing Crosstalk between Linkers}}
\label{subsec-linker-crosstalk}

Our design requires a bit of care with the toeholds. Briefly, each toehold can be equal for any ``high-level species strands'' (such as $A$, $B$, $C$ in Figure \ref{fig:NAND-trimol}), and for any buffer strands. However, to avoid unnecessary ``crosstalk'' between buffers and linkers, and between linkers from two different reactions, it is necessary to use different toehold regions for linkers.

Consider the reactions of Section \ref{subsubsec-NAND}. The first three reactions share a third reactant $\species{0}_o$. This implies that the linker strand of Figure \ref{fig:NAND-trimol} corresponding to these reactions shares the first recognition region $c$ representing $\species{0}_o$. If the toehold $t_i$ following the recognition region were equal for these linker strands, then one linker strand could attach to the gate complex $g_1$ of another reaction, erroneously displacing the strand representing $\species{0}_o$. To prevent this we use different toeholds for each of these reactions that share their third reactant $\species{0}_o$. Similarly, to prevent linkers from displacing non-final reactants (first reactants in a bimolecular reaction, and first or second reactants in a termolecular reaction), we must ensure that $t_i \neq t$ for any $i\in\{1,2,3\}$.

This applies to bimolecular high-level reactions as well, but it is routine to verify that no more than three different reactions (the worst case being the case described above) share the same final reactant. It is safe to reuse linker toeholds between reactions that differ in their final reactant because the different initial recognition regions on the linkers will prevent the crosstalk problem described above.

\opt{dnasubmission}{
\subsection{Preventing Crosstalk between Buffers}}
\opt{normal}{
\subsubsection{Preventing Crosstalk between Buffers}}
\label{subsec-buffer-crosstalk}

Although we have ensured that buffers and linkers will not have crosstalk because they use different toehold sequences, we must ensure that buffers do not suffer undesired crosstalk with each other.  A buffer, unlike a linker, when released uncovers a toehold that is intended to serve as an initial binding site for a strand. Therefore it is not as simple as changing the toehold to prevent buffer crosstalk. Also, a buffer1 strand (a buffer released upon the binding of a first reactant in a reaction, either bimolecular or termolecular) is not garbage-collected as a buffer2 strand is (a buffer released upon the binding of a second reactant in a termolecular reaction). Therefore we must ensure that buffer1 strands are always different from buffer2 strands so that exactly the buffer2 strands are garbage-collected.

To see that this undesired crosstalk does not happen, it suffices to inspect the order of reactants in each reaction. No ``high-level species'' (corresponding to $A$, $B$, etc. in Figures \ref{fig:NAND-bimol} and \ref{fig:NAND-trimol}) is a first reactant in one bimolecular or termolecular reaction but a second reactant in another termolecular reactant. Therefore it is critical to maintain the specific order of the reactants we chose for the high-level reactions of Section \ref{subsec-abstract-CRN-for-gates}. 
